Harnessing Large Language Models for Knowledge Graph Question Answering via Adaptive Multi-Aspect Retrieval-Augmentation

Large Language Models (LLMs) demonstrate remarkable capabilities, yet struggle with hallucination and outdated knowledge when tasked with complex knowledge reasoning, resulting in factually incorrect outputs. Previous studies have attempted to mitigate it by retrieving factual knowledge from large-scale knowledge graphs (KGs) to assist LLMs in logical reasoning and prediction of answers. However, this kind of approach often introduces noise and irrelevant data, especially in situations with extensive context from multiple knowledge aspects. In this way, LLM attention can be potentially mislead from question and relevant information. In our study, we introduce an Adaptive Multi-Aspect Retrieval-augmented over KGs (Amar) framework. This method retrieves knowledge including entities, relations, and subgraphs, and converts each piece of retrieved text into prompt embeddings. The Amar framework comprises two key sub-components: 1) a self-alignment module that aligns commonalities among entities, relations, and subgraphs to enhance retrieved text, thereby reducing noise interference; 2) a relevance gating module that employs a soft gate to learn the relevance score between question and multi-aspect retrieved data, to determine which information should be used to enhance LLMs' output, or even filtered altogether. Our method has achieved state-of-the-art performance on two common datasets, WebQSP and CWQ, showing a 1.9\% improvement in accuracy over its best competitor and a 6.6\% improvement in logical form generation over a method that directly uses retrieved text as context prompts. These results demonstrate the effectiveness of Amar in improving the reasoning of LLMs.

==> checklist.tex <==
\section{Reproducibility Checklist}
This paper:
\begin{itemize}
\item Includes a conceptual outline and/or pseudocode description of AI methods introduced. yes
\item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. yes
\item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. yes
\end{itemize}

\noindent Does this paper make theoretical contributions?  no

\noindent Does this paper rely on one or more datasets? yes

\noindent If yes, please complete the list below.
\begin{itemize}
\item A motivation is given for why the experiments are conducted on the selected datasets. yes 
\item All novel datasets introduced in this paper are included in a data appendix. NA
\item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. NA
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. yes
\item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. yes
\item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. NA
\end{itemize}

\noindent Does this paper include computational experiments? yes

\noindent If yes, please complete the list below.
\begin{itemize}
\item Any code required for pre-processing data is included in the appendix. yes
\item All source code required for conducting and analyzing the experiments is included in a code appendix. yes
\item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. yes
\item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from. yes
\item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. yes
\item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. yes
\item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. yes
\item This paper states the number of algorithm runs used to compute each reported result. yes
\item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. yes
\item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). yes
\item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. yes
\item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. yes
\end{itemize}
